Leveraging Synthetic Audio Data for End-to-End Low-Resource Speech Translation

This paper describes our system submission to the International Conference on Spoken Language Translation (IWSLT 2024) for Irish-to-English speech translation. We built end-to-end systems based on Whisper, and employed a number of data augmentation techniques, such as speech back-translation and noise augmentation. We investigate the effect of using synthetic audio data and discuss several methods for enriching signal diversity.

==> tables/old.tex <==
\begin{table*}[thp]
\centering
\begin{footnotesize}
\begin{tabular}{@{}cclcccccc@{}}
\toprule
\textbf{Whisper} & \textbf{Model} & \multicolumn{1}{c}{\textbf{Datasets}} & \textbf{Data Size} & \textbf{BLEU ↑} & \textbf{ChrF++ ↑} & \textbf{WER ↓} & \textbf{Semantic 1 ↑} & \textbf{Semantic 2 ↑} \\ \midrule
Small & A & authentic & 29,663 & 30.58 & 47.28 & 59.66 & 61.05 & 62.87 \\
Small & B & A + synthetic & 48,719 & 29.54 & \textbf{50.01} & 64.07 & 63.27 & 64.84 \\
Small & C & B + augmented & 146,157 & \textbf{32.91} & {\ul 49.96} & \textbf{57.68} & \textbf{63.78} & \textbf{65.04} \\ \midrule
Medium & D & B + augmented & 146,157 & 35.35 & 52.55 & 54.43 & 65.83 & 67.18 \\ \midrule
Large & E & B + augmented & 146,157 & 35.54 & 52.43 & 53.76 & 67.25 & 68.35 \\ \bottomrule
\end{tabular}
\end{footnotesize}
\caption{Evaluation Results: Model C fine-tuned on both authentic and synthetic data as well as two versions of augmentation (low-amplitude sample removal and noise injection) achieves improvements across all metrics.}
\end{table*}
